Decentralized Online Big Data Classification - a Bandit Framework

Distributed, online data mining systems have emerged as a result of applications requiring analysis of large amounts of correlated and high-dimensional data produced by multiple distributed data sources. We propose a distributed online data classification framework where data is gathered by distributed data sources and processed by a heterogeneous set of distributed learners which learn online, at run-time, how to classify the different data streams either by using their locally available classification functions or by helping each other by classifying each other's data. Importantly, since the data is gathered at different locations, sending the data to another learner to process incurs additional costs such as delays, and hence this will be only beneficial if the benefits obtained from a better classification will exceed the costs. We assume that the classification functions available to each processing element are fixed, but their prediction accuracy for various types of incoming data are unknown and can change dynamically over time, and thus they need to be learned online. We model the problem of joint classification by the distributed and heterogeneous learners from multiple data sources as a distributed contextual bandit problem where each data is characterized by a specific context. We develop distributed online learning algorithms for which we can prove that they have sublinear regret. Compared to prior work in distributed online data mining, our work is the first to provide analytic regret results characterizing the performance of the proposed algorithms.

==> cascaded.tex <==
\section{Online Learning in Cascaded Classifier Systems}

Different from the previous sections, in this section I assume that the classifiers are cascaded. The goal is to make a correct classification in a delay sensitive environment. When an input data stream arrives, it is forwarded to one of ${\cal M}$ classifiers. The classifier has three options. It can label the data as {\em classified} and return the label, label it as {\em irrelevant} and discard it, or label it as {\em further investigation is needed} and send it to another classifier. 

The goal is to learn which classification order is optimal for each arriving data $x(t)$. Note that there are $M!$ classification orders for each data, therefore even the optimization problem is very difficult to solve. However, it can be solved easily in an online setting. The learning algorithm choses an order $\sigma(1), \sigma(2), \ldots, \sigma(M)$ at each time step. For instance assume that for data input $x$, $\sigma(1), \sigma(2)$ is an optimal order. After a {\em classified} decision by the second classifier in the chain, the server not only updates the reward of the classification order $\sigma(1), \sigma(2), \ldots, \sigma(M)$, but it can update the rewards of all classification orders starting with $\sigma(1), \sigma(2)$. If you think of each arm as a classification order, then this learning problem exploits the correlation between the arms. I also propose to use a zooming type algorithm here. By this we don't have to worry about how the data arrives. 

We can also explore more complex classifier structures such as chains of classifiers working in parallel with different input data streams, but they can call each other sometimes to benefit from experience of other classifiers. 

==> centralized.tex <==
\section{An Optimal Classification Scheme with Perfect Information} \label{sec:centralized}

Our benchmark when evaluating the performance of the learning algorithms is the optimal distributed solution which is computed offline given the complete knowledge about the data arrival process and classifier accuracies. 
%For simplicity, we focus on the distributed classification problem of classifier $i$ 
In the optimal classification scheme, for each context $x \in {\cal X}$ classifier $i$ wants to find the optimal classification function from the set $\cup_{i \in {\cal M}} {\cal F}_i$, i.e., the classification function $k$ with the highest accuracy minus the cost of classification $d_k$. We assume that the context space and classification accuracies have the following structural property:
%
\begin{assumption} \label{ass:lipschitz}
For each $k \in \cup_{i \in {\cal M}} {\cal F}_i$, there exists $L>0$, $\alpha>0$ such that for all $x,x' \in {\cal X}$
%
\begin{align*}
|\pi_k(x) - \pi_k(x')| \leq L |x-x'|^\alpha.
\end{align*}
%
\end{assumption}
%
Assumption \ref{ass:lipschitz} indicates that the accuracy of a classifier for similar contexts will be similar to each other. For example, when the context is the time of the day, population density which affects the classifier accuracy at times $x$ and $x'$ will be close to each other when the times $x$ and $x'$ are close to each other. Therefore the relation between classifier accuracy and time can be written down as a Lipschitz condition.  


\rev{For a set $A$ let $|A|$ denote the cardinality of that set.} In this section, we assume that the optimal classification scheme for any classifier $i$ 
partitions ${\cal X}$ into  $|\cup_{i \in {\cal M}} {\cal F}_i|$ sets in each of which a single classification function is optimal.
%Note that partitioning $[-1,1]^d$ is not enough because the noise can carry a data point outside of $[-1,1]^d$.
In order to solve this problem exactly, classifier $i$ needs to know the classification function that yields the \rev{lowest expected cost} for each $x \in {\cal X}$, which is computationally intractable. Assume for an instance that everything is known. Classifier $i$ has access to all classification functions $\cup_{i \in {\cal M}} {\cal F}_i$ and it knows $q_i$. Then the optimal solution for classifier $i$ is given by the following optimization problem.  
%
\begin{problem}\label{prob:opt}
When the classifier accuracies for each context $x \in {\cal X}$ is completely known, the optimal classification regions
%
\begin{align*}
{\cal R}^* = \{R^*_k\}_{(k \in \cup_{i \in {\cal M}} {\cal F}_i)},
\end{align*}
%
of ${\cal X}$ are the solution of 
%
\begin{align}
\textrm{{\bf (P1)  }} {\cal R}^* = \argmin_{{\cal R} \in \Theta} E \left[ \left| Y - \sum_{k \in \cup_{i \in {\cal M}} {\cal F}_i} k(X) I(X \in R_l) \right| + \sum_{k \in {\cal F}_i} d_k I(X \in R_k) + \sum_{k \in {\cal M}_{-i}}  d_k I \left(X \in \cup_{j \in {\cal F}_k} R_j \right)   \right], \label{eqn:opt}
\end{align}
%
where $\Theta$ is the set of $|\cup_{i \in {\cal M}} {\cal F}_i|$-set partitions of ${\cal X}$, the expectation is taken with respect to the distribution $q_i$ and $Y$ is the random variable denoting the true label. Here $I(X \in R_l)$ denotes the event that data received by the classifier belongs to the $l$th set of the partition ${\cal R}$ of ${\cal X}$.
%
\end{problem}

Note that ${\cal R}^*$ depends on $d_k$. Although, we made no assumptions on $d_k$s, in general exchanging data and label with other classifiers is more costly for a classifier then using its own classification function. Therefore without loss of generality we can assume that $d_l > d_k$ for $l \in {\cal M}_{-i}$, $k \in {\cal F}_i$.
%
The complexity of finding the optimal classification regions increases exponentially with $|\cup_{i \in {\cal M}} {\cal F}_i|$. The learning problem we are trying to solve is even harder because the classifiers are distributed, so each classifier cannot directly access to all classifier functions (classifier $i$ only knows set ${\cal F}_i$ and ${\cal M}$, but it does not know any ${\cal F}_j, j \in {\cal M}_{-i}$), and the distributions $q_i$, $i \in {\cal M}$ are unknown. Therefore, we need to use online learning techniques that does not rely on solving the optimization problem in given (\ref{eqn:opt}) or an estimated version of it. 
